Q-STAR:A Perceptual Video Quality Model Considering Impact of Spatial, Temporal, and Amplitude Resolutions

In this paper, we investigate the impact of spatial, temporal and amplitude resolution (STAR) on the perceptual quality of a compressed video. Subjective quality tests were carried out on a mobile device. Seven source sequences are included in the tests and for each source sequence we have 27 test configurations generated by JSVM encoder (3 QP levels, 3 spatial resolutions, and 3 temporal resolutions), resulting a total of 189 processed video sequences (PVSs). Videos coded at different spatial resolutions are displayed at the full screen size of the mobile platform. Subjective data reveal that the impact of spatial resolution (SR), temporal resolution (TR) and quantization stepsize (QS) can each be captured by a function with a single content-dependent parameter. The joint impact of SR, TR and QS can be accurately modeled by the product of these three functions with only three parameters. We further find that the quality decay rates with SR and QS, respectively are independent of TR, and likewise, the decay rate with TR is independent of SR and QS, respectively. However, there is a significant interaction between the effects of SR and QS. The overall quality model is further validated on five other datasets with very high accuracy. The complete model correlates well with the subjective ratings with a Pearson Correlation Coefficient (PCC) of 0.991.

==> abstract_intro.tex <==
\begin{abstract}
In this paper, we investigate the impact of spatial, temporal and amplitude resolution (STAR) on the perceptual quality of a compressed video. Subjective quality tests were
carried out on a mobile device. Seven source sequences are included in the tests and for each source sequence we have 27 test configurations generated by JSVM encoder (3 QP levels, 3 spatial resolutions, and 3 temporal resolutions), resulting a total of 189 processed video sequences (PVSs). Videos coded at different spatial resolutions are displayed at the full screen size of the mobile platform. Subjective data reveal that the impact of spatial resolution (SR), temporal resolution (TR) and quantization stepsize (QS) can each be captured by a function with a single content-dependent parameter. The joint impact of SR, TR and QS can be accurately modeled by the product of these three functions with only three parameters. We further find that the quality decay rates with SR and QS, respectively are independent of TR, and likewise, the decay rate with TR is independent of SR and QS, respectively. However, there is a significant interaction between the effects of SR and QS. The overall quality model is further validated on five other datasets with very high accuracy. The complete model correlates well with the subjective ratings with a Pearson Correlation Coefficient (PCC) of $0.991$. We also conduct the quality comparison between scalable videos coded using H.264/SVC and non-scalable video produced by H.264/AVC, under the same STAR, using paired comparison. The result shows that the proposed QSTAR model is applicable to both scalable and non-scalable video.

%From the model and subjective tests, we found an one-parameter inverted exponential dropping trend
%can be applied to the perceptual quality regarding the spatial resolution and quantization stepsize,
%while the perceptual quality dropping rate against spatial resolution is affected by the quantization
%stepsizes for the same video content.
\end{abstract}
% IEEEtran.cls defaults to using nonbold math in the Abstract.
% This preserves the distinction between vectors and scalars. However,
% if the conference you are submitting to favors bold math in the abstract,
% then you can use LaTeX's standard command \boldmath at the very start
% of the abstract to achieve this. Many IEEE journals/conferences frown on
% math in the abstract anyway.

% no keywords
\begin{keywords}
Perceptual video quality, quality model, spatial resolution, quantization, frame rate, scalable video
\end{keywords}



% For peer review papers, you can put extra information on the cover
% page as needed:
% \ifCLASSOPTIONpeerreview
% \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% \fi
%
% For peerreview papers, this IEEEtran command inserts a page break and
% creates the second title. It will be ignored for other modes.
%\IEEEpeerreviewmaketitle



\section{Introduction}\label{sec:intro}
%\PARstart{V}ideo transmission over wireless networks, such as WiFi, 3G, or 4G, is nowadays getting more prevalent for users to share informations among their social networks, especially on mobile platform.
\PARstart{N}{etworked} video applications such as streaming and chat are becoming prevalent, especially over wireless networks and using small mobile devices.
The users in such application are very heterogeneous in their access link bandwidth, processing and display capabilities. The primary parameters of a video bitstream, which control the
bandwidth requirement, include quantization stepsize (QS) (controlling amplitude resolution), frame rate (controlling temporal resolution or TR)
and frame size (controlling spatial resolution or SR). Given the bandwidth limitation and display resolution of a receiver, the encoder, a network transcoder or adaptor has to decide at which spatial, temporal,
and amplitude resolution (STAR) to code, transcode or adapt a video, to achieve
the best perceptual quality. Therefore, it is important to understand the
impact of the STAR on the perceptual quality. On the other hand, studying the joint impact of
all three dimensions on the perceptual quality is a complex and challenging task.

Some prior works e.g.,~\cite{frameVSquantization,Hauske03subjectiveimage,QualityMetricTQuantBitRate, Lee_VideoQualityExperience, cheon, demin, CrossDQualtiyLowBitVideo, Elsevier_08_HWu}, have explored the impact of SR, TR and quantization artifacts (not QS directly) fully or partially on perceived video quality. Among them,~\cite{frameVSquantization} considers the tradeoff between quantization artifacts and frame rate reduction, and the influence of the display environment on this tradeoff. The authors found that high spatial quality is more preferable than high frame rate, but viewers are more sensitive to frame rate reduction for mobile than desktop devices. In~\cite{Hauske03subjectiveimage, QualityMetricTQuantBitRate} authors proposed a video quality metric, which is a wighted sum of two terms, one is PSNR of the interpolated sequences from the original low frame-rate video and another one is frame-rate reduction. However, \cite{Hauske03subjectiveimage} uses constant values and~\cite{QualityMetricTQuantBitRate} uses motion of the sequences as weighting factors. In~\cite{Elsevier_08_HWu} authors proposed to model the quality of a video with varying frame rate as the product of a function of the  frame rate and a function of the QS, which is quite close to our proposed model (when the SR is fixed) conceptually. However they assume the first function is linear with the frame rate, which does not capture the effect of frame rate accurately based on our subjective test results. The second function decays exponentially with the QS, similar to our earlier model for the quantization effect~\cite{yao2}.

Authors in~\cite{demin, cheon, Lee_VideoQualityExperience, CrossDQualtiyLowBitVideo} further consider the influences of spatial resolution on perceived quality. The quality model in~\cite{Lee_VideoQualityExperience} is a function of the bitrate and a so called truncated bitrate ratio of SNR-scalability, while the quality model in~\cite{cheon}, similar to the work in~\cite{Hauske03subjectiveimage}, is a function of PSNR, TR and SR.
Although the quality assessment in~\cite{cheon,demin} include 3 and 6 different spatial resolutions, respectively, these works only involve an SR range from QCIF to CIF. The works in~\cite{Lee_VideoQualityExperience,CrossDQualtiyLowBitVideo} only include two SR's, QCIF and CIF. Furthermore, none of the tests reported in~\cite{demin, cheon, Lee_VideoQualityExperience, CrossDQualtiyLowBitVideo} were carried out on mobile devices. Even though the work in~\cite{Hauske03subjectiveimage} is for mobile devices, authors assumed that model parameters are independent of video content, while on the contrary, authors in~\cite{Elsevier_08_HWu} believe that the model parameters depend on video contents. Nevertheless,~\cite{Elsevier_08_HWu} does not consider how to estimate the model parameters.

In our previous works~\cite{yenfu_csvt, yao2}, we investigated the impact of TR and QS on perceptual video quality, which was evaluated on larger-screen of laptop monitor, and proposed the video quality model considering the effect of TR and QS under a fixed SR (CIF).
%However, we believe that the form factor and the display screen may affect the viewing experiences. It is important to use a display environment similar to the actual mobile device during the subjective test.  Therefore, in this work, we conduct the test on a mobile platform (Zoom2 from TI) with a screen size of 4.1-inch at a resolution of WVGA (854x480).
In a preliminary study~\cite{yuan_thesis}, we conducted a subjective test to explore the impact of SR and QS, where the subjective tests were done on a mobile platform with small display screen. In this paper, we extend the previous works by considering the interaction of SR, TR, and QS, and propose a complete quality model in terms of SR, TR, and QS. Preliminary results of this study were reported in~\cite{yenfu_ivmsp}. This journal version provides a more comprehensive analysis of the subjective test results, including examining  interaction of the TR, SR, and QS, validating the model with other datasets, and furthermore investigates the quality comparison between scalable videos coded using H.264/SVC and non-scalable videos produced by H.264/AVC.
The remainder of this paper is organized as follows:
Section~\ref{sec:qualitytests} introduces the quality assessment environment, test methodology and data post-processing.
Section~\ref{sec:QSTAR} analyzes the results of subjective tests and present our proposed model. We further study the statistical significance of STAR variables on subjective quality in Sec.~\ref{sec:ANOVA_analysis} and Sec.~\ref{sec:Validation_model} validates the proposed models on other datasets.
%Section~\ref{sec:singlelayer} addresses analytical results of the paired comparison between scalable and non-scalable videos. 
We conclude our work in Section~\ref{sec:conclusion}.
%%--------------------------------------------------------------------
%% Table for acronyms
%%--------------------------------------------------------------------
\begin{table}[htp]
\centering
\caption{List of Acronyms} \label{tab:acronyms}
\begin{tabular}{|l|p{6 cm}|}
 \hline
TR & Temporal resolution\\
SR & Spatial resolution \\
QP & Quantization parameter\\
QS & Quantization stepsize \\
FR & Frame rate \\
PVS & Processed video sequence\\
MOS & Mean opinion score \\
NQT & Normalized quality v.s. normalized temporal resolution\\
NQS & Normalized quality v.s. normalized spatial resolution \\
NQQ & Normalized quality v.s. inverted normalized quantization stepsize\\
MNQQ & Model for NQQ\\
MNQS & Model for NQS \\
MNQT & Model for NQT \\
PCC & Pearson Correlation Coefficient \\
RMSE & Root mean square error\\
 \hline
\end{tabular}
\end{table}

